Exploring and Characterizing Large Language Models For Embedded System Development and Debugging

Large language models (LLMs) have shown remarkable abilities to generate code, however their ability to develop software for embedded systems, which requires cross-domain knowledge of hardware and software has not been studied. In this paper we develop an extensible, open source hardware-in-the-loop framework to systematically evaluate leading LLMs (GPT-3.5, GPT-4, PaLM 2) to assess their capabilities and limitations for embedded system development. We observe through our study that even when these tools fail to produce working code, they consistently generate helpful reasoning about embedded design tasks. We leverage this finding to study how human programmers interact with these tools, and develop an human-AI based software engineering workflow for building embedded systems. Our evaluation platform for verifying LLM generated programs uses sensor actuator pairs for physical evaluation. We compare all three models with N=450 experiments and find surprisingly that GPT-4 especially shows an exceptional level of cross-domain understanding and reasoning, in some cases generating fully correct programs from a single prompt. In N=50 trials, GPT-4 produces functional I2C interfaces 66% of the time. GPT-4 also produces register-level drivers, code for LoRa communication, and context-specific power optimizations for an nRF52 program resulting in over 740x current reduction to 12.2uA. We also characterize the models' limitations to develop a generalizable human-AI workflow for using LLMs in embedded system development. We evaluate our workflow with 15 users including novice and expert programmers. We find that our workflow improves productivity for all users and increases the success rate for building a LoRa environmental sensor from 25% to 100%, including for users with zero hardware or C/C++ experience.

==> sections/autoethnography.tex <==
\section{Auto-Ethnographic Study}

Here we will all play with chatGPT4 based on the findings from motivation section and talk about it. This will be used to generate limitations to test in userstudy. 

==> sections/conclusion.tex <==
\section{Conclusion}
Prior work has demonstrated the ability of advanced LLMs like GPT-4 and Palm 2 have significant cross-domain reasoning abilities, even for situations that have not been explicitly represented in their training data. We find evidence that this reasoning ability extends to the complex relationship between software and hardware that lies at the core of the embedded system development process. Models like GPT-4 are far more than code autocomplete utilities - they are able to rationalize about the behavior of the physical world and produce code to operate hardware that interfaces with it. This has promising implications for future work in the embedded systems community to increase developer productivity in building robust and efficient systems. However, this also comes with profound risks. It is imperative that future work in this area proceeds responsibly and does not lose sight of our responsibility as embedded systems professionals to build ethical and safe systems. 


% conclusion that it is improtant area of future research. Reason across specific situations it has not seen before. Suprising result is we see similar capapbilities on embedded tasks as complex reasoning in other fields. Can do a lot more than code autocomplete. Interfaces with the physical world to produce input and output, somethign we should be careful with, develop respomsibly, etc. Prior work has demonstrated the ability of advanced LLMs like GPT-4 and Palm 2 have significant cross-domain reasoning abilities, and we find evidence that this extends to the complex relationship between software and hardware that lies at the core of the embedded system development process. 

==> sections/intro-1.tex <==
\section{Introduction}
Large language models (LLMs) such as GPT-3.5, GPT-4 and PaLM2 have recently made significant strides in automated code generation for a variety of general software development tasks. These language models, which have been trained on many code samples, have proven to be capable of generating syntactically correct and semantically meaningful code, in response to high-level task descriptions, which rivals human experts on certain tasks~\cite{bubeck2023sparks}. Researchers have also begun to explore numerous methods of improving the base models for software development tasks such as methods of encoding user intent~\cite{lahiri2022interactive}, self-repair for automated debugging allowing models to correct their own mistakes~\cite{olausson2023demystifying}, and self-collaboration between multiple LLMs~\cite{dong2023selfcollaboration}. Commercially available integrated development environments (IDEs) have already begun to incorporate these tools~\cite{copilot1} suggesting that AI assistants will play a growing role in software development workflows in years to come.

Despite significant effort in using LLMs for general software engineering, there has been little to no study of their use for embedded systems development. Embedded systems design and programming differs from general purpose software development in that it requires cross-domain understanding of not only the software but also hardware and how it interacts with the physical world~\cite{wolf2010high,lee2011introduction}. For example, even designing a simple wireless sensor node measuring a quantity like temperature requires complex reasoning and understanding about each of the chips, their registers and operating modes, communication protocols between the chips and the network, power consumption, as well as understanding and verifying the physical signals. This raises the question, can LLMs understand and reason about these concepts and can they play an effective role in embedded system development?

In this paper, we conduct an exploratory analysis of the performance of leading large-language models (GPT-3.5 \cite{TODO}, GPT-4 \cite{openai2023gpt4}, and PaLM 2~\cite{anil2023palm}) on embedded system development tasks with the goal of understanding their behavior and developing actionable use cases. We perform a systematic investigation studying the performance of LLMs on a suite of embedded system design tasks and concepts including code generation, hardware understanding, debugging, and system design optimization. We find to our surprise that GPT-4 in particular demonstrates an exceptional level of cross-domain understanding and reasoning ability, including inter-chip and wireless communication protocols, hardware components, and application design spaces. We even observe it generate register-level drivers for common Integrated Circuits (ICs). We also observe and characterize the models' limitations which differ from human programmers and propose solutions. In addition to individual tests, we develop physical test benches consisting of sensor-actuator pairs to perform real-time testing of the code output on development boards to compare models and serve as a tool for future model tuning. We synthesize these findings into a generalizable workflow for using LLMs in embedded system software development and evaluate it with a user study to understand how LLMs can benefit both novice and expert programmers.

To evaluate the capabilities of LLMs for embedded system design, we first seek to compare the performance of openly available high performance models on a common set of benchmark tasks. Designing such a benchmark however raises an important question, how can we programmatically verify that an LLM generates valid code? While simple text generation programs can be verified with print statements, we seek to go a step further and probe LLMs' abilities to generate code for end-to-end systems that interacts with the physical world through sensors. End-to-end testing requires a means to induce and measure physical stimuli, while also accounting for environmental noise. We prototype and evaluate a set of physical testbenches consisting of sensor-actuator pairs and an automated data analysis pipeline that compares the output of verified human written code to data from LLM generated code. For example by combining an LED and photodiode or rangefinder and linear actuator we can probe two sensors side-by-side to directly compare the signal sampled by the LLM code and correct human code. This enables robust benchmarking for model comparison with hundreds of trials and establishes a method for future closed-loop testing and model fine tuning.

\begin{figure}[!t]
\centerline{\includegraphics[width=0.35\textwidth]{figures/Github_Number of code.png}}
\vskip -0.2in
\caption{Number of files in different languages on Github showing that embedded systems code is likely less represented than other software.}
\vskip -0.2in
\label{fig:github_code_files}
\end{figure}

\textcolor{red}{TODO: maybe this paragraph is a good place to mention the amount of Arduino code}
The strong performance of models such as GPT-4 on our code generation testbench demonstrates that LLMs can successfully generate end-to-end embedded systems code; however this raises many questions about what knowledge the models actually have and how well they can generalize to other tasks. For instance, even the simplest ``hello world'' program for embedded systems, like blinking an LED, requires understanding of both the software and hardware. This includes understanding the need to initialize GPIO pins and correctly configuring them to drive an output, manipulating them to set the pin on and off as well as understanding how this affects the LED, as well as the physical hardware connections.
Considering these models are trained on text scraped from the Internet, we took a brief look at one large source of code examples part of this training dataset: GitHub, an online service for hosting code repositories.
As can be seen in Figure~\ref{fig:github_code_files}, the distribution of code examples that these models have been trained on lean heavily towards programming languages used in traditional software applications, such as JavaScript and Python.
On the other hand, the amount of training examples relevant for embedded systems development, such as Arduino and a subset of C and C++, is orders of magnitudes smaller.
As a result, since these models are not specifically fine tuned for the embedded systems domain, it is unclear whether they have robust knowledge of these topics or the cross-domain reasoning ability to solve problems in this space.

We perform a series of experiments to systematically probe the models to study their understanding of the hardware itself, embedded systems specific software design concepts such as interrupts, and high level design and debugging advice. We design a series of prompts asking the model to generate code for interfacing with sensors and peripherals. We find surprisingly that GPT-4 has a detailed understanding of numerous ICs down to individual register addresses and operating modes. Moreover, the model is able to correctly construct programs using these register maps to perform high level tasks and generate disclaimers noting that it does not have access to updated information beyond its training data cutoff in 2021. Additionally, we design a custom register table to evaluate the model's response to data outside of its training set. We further observe that similar to other software engineering tasks, the models can easily generate a program structure, call external libraries, and perform self-repair. We also find that GPT-4 is capable of providing both software and hardware debugging advice on checking physical connections and more.

During this process we also observe a number of limitations and errors. We note that a number of these are consistent with programming errors observed in other domains such as hallucinations and trouble with specific numbers. We categorize these errors and suggest solutions to each. We synthesize these findings into a generalizable workflow for using LLMs in embedded system software development and perform a user study with 15~participants ranging from zero programming experience to experienced designers.

We summarize our contributions and key findings below:
\textcolor{red}{TODO: remove indentation from this. Maybe revise this as well and add some numbers depending on the results?}
\joe{maybe these contributions should also be in the same order that they are presented in the paper? i.e. evaluation/test-bed framework goes first?}
\squishlist
    \item \joe{contribution should be made more concrete}\zach{I agree} We perform a systematic analysis of LLMs for a variety of embedded systems tasks. We find the surprising result that LLMs such as GPT-4 which are not optimized for embedded systems development demonstrate significant cross-domain understanding and reasoning of both hardware and software. However, we also observe many errors are common issues seen in LLM code generation such as trouble with numbers and hallucinations, as well as domain specific problems like effectively encoding the system's state for the model.
    \item We construct a set of physical testing platforms, each consisting of sensors-actuators pairs for programmatic real-time code evaluation and further hardware-in-the-loop model refinement. We perform a series of experiments (N=450) comparing different models and find GPT-4 outputs correct code \textcolor{red}{XXX\% of the time.}
    \item Leveraging these findings, we develop a set of prompting strategies and propose an AI integrated development workflow for embedded systems design, programming and debugging.
    \item We conduct a user study of constructing end-to-end wireless IoT nodes and receivers with 15 participants of varying skill levels.  We observe that experienced users express high satisfaction and that participants with \textit{zero} C/C++ programming or electronics hardware experience can build a fully functioning LoRa-based environmental sensor in just 40 minutes with GPT-4's programming and debugging assistance.
\squishend

\textcolor{red}{TODO: does this relate to other points above?}We provide a comprehensive analysis of tasks for developing wireless sensor nodes and reveal both capabilities and limitations, including an open dataset of chat logs.


==> sections/intro-2.tex <==
\section{Introduction}
Large language models (LLMs) such as GPT-3.5, GPT-4 and PaLM 2 have recently made significant strides in code generation for a variety of software development tasks. These LLMs, which have been trained on many code samples, can generate syntactically correct and semantically meaningful code from high-level task descriptions, and rival human experts on certain tasks~\cite{bubeck2023sparks}. Researchers have also begun exploring optimizations such as encoding user intent~\cite{lahiri2022interactive}, self-repair for LLMs to correct their mistakes~\cite{olausson2023demystifying}, and self-collaboration between multiple models~\cite{dong2023selfcollaboration}. Commercially available integrated development environments (IDEs) have already begun to incorporate these tools~\cite{copilot1} suggesting that AI assistants will play a growing role in software development workflows in years to come.

\begin{figure}[!t]
\centerline{\includegraphics[width=0.9\textwidth]{figures/Overview.pdf}}
\vskip -0.2in
\caption{Illustration of human AI co-design for embedded system development with our automated hardware-in-the-loop testing framework.}
\label{fig:overview}
\vskip -0.3in
\end{figure}

Despite these efforts, there has been little to no study of using LLMs for embedded systems development. For example, while tools like Github Co-Pilot can auto-complete code, they have no link to the hardware, no context about the interconnections of components in the system, or what outputs they would produce. Embedded systems design and programming straddles the hardware-software interface and requires a cross-domain understanding of how devices \textit{interact with the physical world}~\cite{wolf2010high,lee2011introduction}. 
Development of embedded systems typically requires a cyclical process of continuous development and verification, entailing numerous software-hardware integration trials. This iterative approach stands in contrast to conventional programming tasks, where outputs are deterministic and predictable. Embedded system development, on the other hand, demands a complex, multi-step reasoning and verification protocol to ensure system reliability and functionality. For example, designing a simple wireless temperature sensor requires a physical understanding of the chips and their interfaces, network connectivity, and the sensed signals. These differences from conventional software development impose a high barrier for human programmers and have inspired projects such as the MakeCode platform focused specifically on improving accessibility to embedded systems development~\cite{karvinen2019lowering,devine2019makecode}. This raises a key question: can LLMs generate reasoning about these concepts, and how can they play an effective role in embedded system development?

In this work we conduct an exploratory analysis of leading large-language models (GPT-3.5 \cite{gpt-3.5}, GPT-4 \cite{openai2023gpt4}, and PaLM 2~\cite{anil2023palm}) on embedded system development and debugging tasks and develop concrete strategies to effectively use them. To enable systematic and repeatable experiments, we design physical interfaces for LLMs to directly interact with physical hardware and create an end-to-end hardware-in-the-loop (HIL) evaluation platform for evaluating LLM generated code. We aim to understand their capabilities and limits, and then develop actionable insights toward workflows in which human programmers co-develop systems with hardware-in-the-loop AI tools as envisioned in Figure~\ref{fig:overview}. 

Using LLMs for embedded systems development raises a number of fundamental questions and challenges. First, to systematically evaluate their performance, how can we programmatically verify that an LLM generates valid code? Such experiments with repeated trials are essential to advance our understanding in this domain beyond blog posts with a handful of experiments; however unlike programs with text output that can be verified with string comparisons, we seek to probe LLMs' abilities to generate code for end-to-end systems that interact with the physical world through sensors. This requires a method of inducing and measuring real-world stimuli, as well as validating the sensor output signals the presence of environmental noise. A robust benchmarking tool and verification pipeline to test LLM generated code for embedded systems is also the first step toward further model optimization through fine-tuning and developing self-repair techniques with hardware in the loop.

Second, using LLMs for hardware-software co-design is still under-explored. Using LLMs with embedded systems raises fundamental questions about the ability of these models to reason about the interaction between hardware,  software, and the physical and digital environments where systems are deployed. Their strong performance on code generation likely results from their training on vast amounts of code available from sources such as Github. We observe however that within this dataset, embedded systems code is poorly represented. Figure~\ref{fig:github_code_files} shows a distribution of file extensions on Github which leans heavily towards JavaScript and Python while embedded systems code, such as Arduino\footnote{Arduino is just one example of a popular platform with a unique filename} and a subset of C and C++, is orders of magnitude smaller. 

Furthermore, developing embedded systems requires both context about how hardware interacts with the physical world, and connecting these concepts to the code itself. For example, even the simple task of "Write a program that blinks an LED" requires an understanding of how components are connected (the correct output pin) and that setting the pin value to a logic level high will produce light. Given that these models are not developed for the domain of embedded systems, there is an element of uncertainty regarding the capacity of task-specific code-generation models, such as Github Copilot, to comprehend and effectively engage with the intricacies of embedded systems interfacing with the physical world. On the other hand, general-purpose models may have a robust representation of these topics or the cross-domain reasoning ability to solve problems in this space.

To address these challenges we begin by developing methods to physically interface microcontroller and sensor outputs with LLMs and create an HIL evaluation platform for systematically verifying programs using sensor actuator pairs. We compare all three models with N=450 experiments and find surprisingly that GPT-4 especially shows  an exceptional level of cross-domain understanding and reasoning, in some cases generating fully correct programs from a single prompt. We perform a series of systematic evaluations probing a variety of embedded system development capabilities and find it generates register-level drivers, I2C interfaces, LoRa communication code, and even suggests specific and actionable methods to power optimize code. During these experiments we make the accidental and surprising discovery that the models can also suggest context-specific hardware debugging advice down to the level of checking wiring.

We also observe and systematically document a number of limitations and errors. For example, on the most complex tasks like asking the model to generate a complete program to read an I2C accelerometer and print the data to serial, only 14\% of programs worked end-to-end even on the best performing model (GPT-4, N=50 trials). We perform an error analysis and observe that even partially correct programs often had significant amounts of functional code, as well as detailed comments and explanation of how to correctly design the system. The reasoning generated has significant potential to help a human developer. Additionally we observe many errors produced by the model could be easily spotted by a human developer such as importing one version of a library but calling functions from another. 

These findings suggest that while LLMs may play a role in fully automated code generation, perhaps more powerful is a new human-AI co-development approach to embedded systems development that combines human context about the system and high level design objectives with LLM code generation abilities. We synthesize these findings into a generalizable workflow to enable human-AI co-development for embedded system software development. We evaluate this workflow through a user study with 15~participants ranging from zero hardware experience to expert designers with 10+ years of experience. We observe that LLMs can benefit expert programmers, however the most dramatic benefits are to novice users. The combination of bridging the gap between high level objectives and low level hardware implementation as well as personalized debugging advice allowed first time embedded programmers to design fully functional systems in as little as 40~min. This human-AI approach has the potential to transform embedded systems education and help reduce the barrier for researchers in the broader Ubicomp community to work on hardware and physical computing topics.

\begin{figure}[!t]
\centerline{\includegraphics[width=0.5\textwidth]{figures/github_code.pdf}}
\vskip -0.2in
\caption{Number of files in different languages on Github showing that embedded systems code is likely less represented than other software.}
\vskip -0.2in
\label{fig:github_code_files}
\end{figure}


%For example, a blink program requires initializing GPIO pins and correctly configure them to drive output, manipulating them to set the pin on and off as well as understanding how this affects the LED, and physically connecting the LED with the correct polarity to produce a working system. 
%We design a series of prompts asking the model to generate code for interfacing with sensors and peripherals. We find surprisingly that GPT-4 has a detailed understanding of numerous ICs down to individual register addresses and operating modes. Moreover, the model is able to correctly construct programs using these register maps to perform high level tasks and generate disclaimers noting that it does not have access to updated information beyond its training data cutoff in 2021. Additionally, we design a custom register table to evaluate the model's response to data outside of its training set. We further observe that similar to other software engineering tasks, the models can easily generate a program structure, call external libraries, and perform self-repair. We also find that GPT-4 is capable of providing both software and hardware debugging advice on checking physical connections and more.

%During this process we also observe a number of limitations and errors. We note that a number of these are consistent with programming errors observed in other domains such as hallucinations and trouble with specific numbers. We categorize these errors and suggest solutions to each. We synthesize these findings into a generalizable workflow for using LLMs in embedded system software development and perform a user study with 15~participants ranging from zero programming experience to experienced designers.

%To answer these questions we design an end-to-end testing perform and perform experiments on ATmega328P (Arduino) and nRF52 MCUs to systematically probe the models to study their performance, understanding of hardware, and develop a workflow to use LLMs for embedded systems development and debugging. 
We summarize our contributions below: 
\squishlist
    % \item We perform a systematic analysis of LLMs for a variety of embedded systems tasks. We find the surprising result that LLMs such as GPT-4 which are not optimized for embedded systems development demonstrate significant cross-domain understanding and reasoning of both hardware and software. However, we also observe many errors are common issues seen in LLM code generation such as trouble with numbers and hallucinations, as well as domain specific problems like effectively encoding the system's state for the model.
    \item \textbf{Physical Testbench.} We build the first open-source, extensible software-hardware evaluation framework for Human-AI embedded system development. It includes an end-to-end pipeline to enable real-time LLM-powered embedded system code generation with sensor-actutor pairs. We support a series of state-of-the-art LLMs in our framework, including PaLM-2, GPT-3.5, and GPT-4. To systematically evaluate the robustness of our framework, we have executed a comprehensive suite of 450 real-world evaluations involving integrated software-hardware interactions. The data and code are released in this \textcolor{red}{anonymous Github}\footnote{\textcolor{red}{LINK}}. We envision our framework will serve as a valuable asset for the research community, fostering further exploration and validation of sensor-driven software-hardware systems in ubiquitous computing
    
    
    
    % Overall, we see GPT-4 performs best, generating functional I2C interfaces 66\% of the time with a single prompt on our most complex task. 
    %Our experiments (N=450) show that GPT-4 produces higher quality embedded than other state of the art LLMs. 
    \item \textbf{Exploration.} We perform the first systematic evaluation of LLM facilitated embedded tasks and show they have a rich cross-domain understanding of hardware and software. We find that LLMs can even provide specific and actionable hardware debugging advice about wiring and analyze programs, reducing power consumption on an nRF52 by over 740x to 12.2 \textmu A. We also characterize limitations like hallucinations and representing the system's state.
    % \item We construct a set of physical testing platforms, each consisting of sensors-actuators pairs for programmatic real-time code evaluation and further hardware-in-the-loop model refinement. We perform a series of experiments (N=450) comparing different models and find GPT-4 outputs correct code \textcolor{red}{XXX\% of the time.}
    \item \textbf{LLM-Based Human-AI development workflow.} We observe that LLMs produce detailed comments and explanations of how to design embedded systems as well as context-specific debugging advice. Leveraging these findings, we develop a set of prompting strategies and propose an AI integrated development workflow for embedded systems design, programming and debugging.
    % \item We conduct a user study of constructing end-to-end wireless IoT nodes and receivers with 15 participants of varying skill levels. We observe that experienced users express high satisfaction and that participants with \textit{zero} C/C++ programming or electronics hardware experience can build a fully functioning LoRa-based environmental sensor in just 40 minutes with GPT-4's programming and debugging assistance.
    \item \textbf{User Study.} We evaluate our workflow with 15 users across experience levels. We find our workflow improves productivity for users across all experience levels and increases the success rate on complex tasks from 25\% to 100\%. This allowed users with zero hardware or C/C++ experience to build a fully functional LoRa environmental sensor transmitter and receiver in 40~min, demonstrating the potential of this approach for education and lowering the barrier for working with hardware.
    %We conduct 15 person user study of constructing end-to-end wireless IoT nodes and receivers. We observe that experienced users express high satisfaction and that participants with \textit{zero} embedded experience can build fully functioning LoRa-based environmental sensors in just 40 minutes with GPT-4's programming and debugging assistance.

    
\squishend

% \textcolor{red}{TODO: does this relate to other points above?}We provide a comprehensive analysis of tasks for developing wireless sensor nodes and reveal both capabilities and limitations, including an open dataset of chat logs.


==> sections/intro.tex <==
\section{Introduction}
Paragraph 1: Write about the  success and promise of using large language models for code generation
AI hype, why is embedded code generation hard? Grounding in physical world "multimodal" tasks, critical tasks that must work reliably and precisely, very little training data relative to other languages and frameworks (github code survey fig) \\

Paragraph 2: people haven't done code gen for embedded/hardware stuff \\

Paragraph 3: In this paper we do XXX \\

Paragraph 4: Challenges of code generation for embedded, more detail, specific things (challenge 1, 2, 3) \\
- Embedded development requires multi-modal cross-domain understanding
ex: simplest "hello world" program is blink, requires connecting an LED
- Less defined design space, like asking for facts
- Models aren't optimized for embedded, much more code on github for general purpose programming
- verifying the output


Paragraph 5: Proposed solutions (or maybe just go to contributions, whatever makes more sense)\\

Bulleted list of contributions
1. comprehensive analysis of what models can do? comparing different tools showing what's possible and what limitations are? 2. Developing a new AI based workflow/new embedded software engineering paradigms 3. How to make it better (using tools, DSLs etc)

In this paper we perform an exploratory analysis of leading large-language models (GPT-3.5, GPT-4, PaLM 2) to assess performance on embedded system programming tasks and explore how human programmers interact with these new tools when building systems. We find that GPT-4 demonstrates an exceptional level of hardware understanding, including communication protocols, hardware components, and design application spaces, and is able to synthesize useful embedded code based on this information, going as far as generating register-level drivers for common ICs. We develop a set physical test benches to perform real-time testing of code output from language models on development boards to enable programmatic evaluation of language models for embedded system tasks. 

We conduct a user study on N participants of various skill levels, ranging from no experience with software or electronics hardware to skilled embedded system developers. Users were tasked with building end-to-end wireless IoT nodes and receivers utilizing Bluetooth and LoRa in addition to more basic timer and interrupt tasks. For some tasks users had access to the open internet, simulating a real-world development scenario, while for other tasks users had access to GPT-4 via ChatGPT. Experienced developers expressed high satisfaction when working with GPT-4, expressing that it generated working or nearly-working code that could be more easily adapted to the desired task than example code found online. 

Surprisingly, GPT-4 proved to be a powerful tool in assisting beginners. Participants with no prior programming or hardware experience were able to write functional code and read data from sensors, while experienced programmers without prior hardware experience were able to build fully-functional LoRa-based environmental sensors when using GPT-4. We also find GPT-4 , both generating code fixes to address errors and often correctly identifying when hardware was improperly configured and prompting the user to check connections, move components to different pins, and even going as far as generating custom code to debug hardware connections and instructing users to run and report back results.  

We conclude that large-language models represent a powerful tool for both improving the coding experience of seasoned developers as well as enabling people with limited hardware or even software experience to quickly implement wireless sensors. 


We emphasize that this is an initial exploration of the topic with the goal of challenging the notion that LLMs cannot be used to develop embedded systems and motivate future research within this domain
not comprehensive, only a handful of platforms tested, mention limitations in discussion

show this is immediately accessible to the community, doesn't require knowledge of AI/ML or many GPUs to fine tune models

compare the types of errors made by AI and human programmers

==> sections/old_discussion.tex <==
\section{Discussion and Conclusion}

\noindent \textbf{Findings.}
We find that advanced LLMs, in particular GPT-4, have an extensive understanding of software techniques, hardware principles, and the relationship between program implementation and the resulting behaviors of end-to-end systems. 
% This makes leading LLMs significantly more powerful for embedded tasks than prior models tuned solely for code completion. 
GPT-4's ability to produce code while also suggesting hardware implementations demonstrates that these models embedded a rich multi-modal representation that spans embedded hardware and software systems.
% We find that they are easily steered by experienced developers who are able to clearly and specifically state what they want and how it should be implemented. This manifests itself in a significant increase in productivity as well as user satisfaction. 

% These models also appear to provide a useful multi-modal layer of abstraction across the hardware and software domains associated with embedded systems development. While a driver library provides a simplified interface for communicating with a sensor, GPT-4 takes this a step further by demonstrating an ability to both produce code and suggest hardware implementations required to complete a desired end-to-end task. This was particularly evident in the user study where participants with coding experience but no hardware experience were able to build working systems from individual components. 

While unable to reliably produce working end-to-end systems, these models may significantly increase productivity and satisfaction when given context-rich prompts by experienced embedded developers. Throughout our user study, we were surprised by the ability of LLMs to assist users in debugging across hardware and software. In particular, GPT-4 provided useful debugging steps and identified sources of incorrect behavior (e.g. incorrect physical connections or I2C addresses) for errors not caught at compile time.

% be them incorrect physical connections or software issues like incorrect I2C addresses, function incompatibilities, and other errors that are not caught in the compilation stage of programs. 
% In addition, GPT-4 provided useful debugging steps to assist users in identifying the root cause of system errors, a complicated task that occupies a significant portion of time in the embedded system development process. 

% Based on the results of our exploration and characterization of the capabilities of LLMs, we identify the following promising areas for future work to both improve the performance of LLMs for embedded code generation tasks as well as assist developers in building working end-to-end systems.  
% We identify the following areas for future work to improve the performance of LLMs for embedded code generation, as well as their assistance to developers in building working end-to-end systems.  

\noindent \textbf{Future Work.}
We observe that GPT-4 is often able to identify and improve code based on feedback regarding the behavior of the system. The physical testing setup implemented in this paper can be extended to provide multi-modal improvements. Compile errors and sensor data from failed physical tests could be fed back to the model to iteratively regenerate code until the desired behavior is achieved. 

Additionally, models could be fine-tuned specifically on electronics datasheets, manuals, and specific embedded SDKs. This would likely reduce register and address hallucinations seen in more complex code generation tasks (e.g. implementing an I2C driver for an IMU). Similarly, the querying ability of LLMs may be use to recover external plugins and API used to provide additional context for generated embedded code.
% In contrast with simpler code generation models, this could be particularly powerful when combined with the cross-domain reasoning ability of a model like GPT-4. 
% Similarly, leveraging the ability of models like GPT-4 to automatically query external plugins and APIs in the process of generating responses, and the development of external plugins to provide models with hardware register tables and similar information holds the potential to make significant improvements in performance on these tasks. 

In our user study, participants relied on a chat interface to manually share code and hardware configurations with GPT-4. A future IDE may automate the process of relaying compile and linking error information directly to an LLM. Additionally, an integrated LLM would be able to examine code in real-time and offer suggestions regarding power consumption, data throughput optimization, and design techniques. We envision this as a power teaching tool for novices and a development accelerant for experience embedded engineers.
% Techniques like this could also be powerful teaching tools, providing guidance and explanations that relate to the specific code a user has written instead of generic examples that may be unfamiliar to less experienced developers. 

Finally, leveraging recent work for visual \cite{zhang2023videollama} and sensor \cite{girdhar2023imagebind} embeddings, future work may present techniques to represent hardware configurations and setup in an consistent and unambiguous embedding used by language models to produce more hardware-informed software.
% Another potentially fruitful area of exploration lies in the challenge of system representation. Leveraging recent work developing embeddings for images, video \cite{zhang2023videollama}, and other sensor data \cite{girdhar2023imagebind}, techniques for embedding hardware configurations could be developed. This would provide a consistent and unambiguous description of the specific hardware setup to the language model and likely assist in producing working code that appropriately interfaces with a user's specific hardware implementation.

% \noindent \textbf{Conclusion.} In their current form, LLMs do not come close to replacing experienced embedded system programmers. However, across the board, access to these tools greatly increases the productivity and satisfaction of developers working on embedded programming tasks. However, feedback on fulfillment was more ambiguous, with many participants expressing that the assistance provided by a language model made them feel less responsible for the resulting output. As language models and tools that leverage them continue to grow in terms of capability, it will be critical to define the role of human developers in the process. This is particularly important in cases where embedded systems are used as part of mission-critical subsystems, where ownership and extensive verification of code can have significant safety implications. 
\noindent \textbf{Discussion.} In their current form, LLMs do not come close to replacing experienced embedded programmers. However, access to these tools greatly increases the productivity and satisfaction of developers working on embedded programming tasks. However, feedback on fulfillment was rather ambiguous, with many participants expressing that LLM assistance made them feel less responsible for the resulting outputs. As the capability of language models and tools that leverage them continue to grow, it will be critical to define the role of human developers in the process. This is particularly important in cases where embedded systems are used for mission-critical subsystems, where ownership and extensive verification of code can have significant safety implications. 

Prior work has demonstrated the ability of advanced LLMs, like GPT-4, to have significant cross-domain reasoning abilities. We find evidence that this reasoning extends to the complex relationship between software and hardware that lies at the core of embedded system development. Models like GPT-4 are far more than code auto-complete utilities - they are able to rationalize the behavior of the physical world and produce code to operate hardware that interfaces with it. This has promising implications for future work in the embedded systems community to increase developer productivity in building robust and efficient systems. However, this comes with profound risks: It is imperative that future work proceeds responsibly and does not lose sight of our responsibility, as embedded systems professionals, to build ethical and safe systems. 

% Major interesting takeaways - it is not perfect but significant reasoning capabilities and can be useful with human in the loop. Very steerable by experienced developers who are able to clearly and specifically articulate what they want, and how it should be implemented. Makes people significantly more productive. 
% knowledge of hardware and protocols is still important, you need to know what question to ask and give appropriate context. Abstraction. It provides a useful layer of abstraction on top of base libraries, etc. but in its current state you still need to know what to ask - to produce something that works really well (expert/pro level) you need to know the things well to specifically prompt and get good results

% Future Research
% Fine tuning to develop code and drivers from datasheets to produce a more consistent abstraction experience - datasheet 
% HW in the loop to do multi-shot improvement - automatically fix bugs based on hw feedback, compiler feedback. 
% IDE could automate some of the workflow for compile errors, HW verification, etc.
% Integrating optimization suggestions into IDE 

% representing system to LLM - right now we rely on user description of system. How to embed complete hardware configuration to enable comprehensive reasoning
% Use as a teaching tool 
% Fulfillment and implications for growth of these tools going forward

% right now they don't replace expert programmers, but across the board these tools are greatly increasing productivity with human+ai collaboration


% conclusion that it is improtant area of future research. Reason across specific situations it has not seen before. Suprising result is we see similar capapbilities on embedded tasks as complex reasoning in other fields. Can do a lot more than code autocomplete. Interfaces with the physical world to produce input and output, somethign we should be careful with, develop respomsibly, etc.


==> sections/old_discussion_short_old.tex <==
\section{Discussion and Conclusion}
Our experiments demonstrate LLMs are far more than code auto-complete utilities - they are able to rationalize the behavior of the physical world and produce code to operate the hardware that interfaces with it. 

While unable to reliably produce working end-to-end systems, these models can be can significantly increase productivity and satisfaction when given context-rich prompts by experienced embedded developers. Throughout our user study, we were surprised by the ability of LLMs to assist users in debugging across hardware and software. In particular, GPT-4 provided useful debugging steps and identified sources of incorrect behavior (e.g. incorrect physical connections or I2C addresses) for errors not caught at compile time.

Future work may address LLMs fine tuned on embedded repositories, datasets, and specific embedded SDKS, IDE integrated LLMs, or more refined hardware specification representations. However, in their current form, LLMs do not come close to replacing experienced embedded programmers. Regardless, access to these tools greatly increases the productivity of developers working on embedded programming tasks. 

Importantly, our user-study feedback regarding fulfillment, though generally positive, was at times ambiguous. Some participants expressed that LLM assistance made them feel less responsible for the resulting systems. As the capability of language models and tools that leverage them continue to grow, it will be critical to define the role of human developers in the process. 

This is particularly important in cases where embedded systems are used for mission-critical subsystems, where ownership and extensive verification of code can have significant safety implications. Large language models have the potential to re-imagine how embedded system development and debugging function. However, they come with profound risks: It is imperative that future work proceeds responsibly to address these concerns and does not lose sight of our responsibility, as embedded systems researchers, to build ethical and safe systems.

==> sections/results.tex <==
\section{Results}

here we will talk about the results and show figures of the userstudy. 
